Towards Decentralised Cloud Storage with IPFS: Opportunities, Challenges, and Future Directions

The InterPlanetary File System (IPFS) is a novel decentralised storage architecture, which attempts to provide decentralised cloud storage by building on founding principles of P2P networking and content addressing. IPFS is used by more than 230k peers per week and serves tens of millions of requests per day, which makes it an interesting large-scale operational network to study. While it is used as a building block in several projects and studies, its inner workings, properties, and implications have only been marginally explored in research. Thus, we provide an overview of the IPFS design and its core features, along with the opportunities that it opens as well as the challenges that it faces because of its properties. Overall, IPFS presents an interesting set of characteristics and offers lessons which can help building decentralised systems of the future.

==> sections/applications.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Applications}
\label{sec:applications}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\viet{This could become ``Discussion and Outlook'': several applications for different purposes, though more research and development
on-going}

% Since the Internet is a medium for both synchronous and asynchronous communication between multiple
% hosts, the information needs to be stored at physical locations to be exchanged. For synchronous
% communication, storing information locally on the device is sufficient. However, for the
% asynchronous scenario, the information needs to be buffered before arriving at the recipients, in
% particular when sending larger files. Thus, the storage and processing of files, i.e. file systems,
% are essential building blocks for the Internet.


In order to make use of the properties of a decentralised file system and its opportunities while
also addressing some of the challenges that were discussed in the previous section, various projects
and applications aiming at decentralising the Internet have adopted and integrated IPFS into their
architecture over the years. These projects leverage IPFS for two main purposes: (a) as a 
file storage, which is not controlled and operated by a single entity, and (b) as a means to
disseminate/cache content efficiently in a decentralised manner.

\hl{application ``classes''?}
Usage ideas and examples (with quite some overlap)\footnote{\url{https://docs.ipfs.io/concepts/usage-ideas-examples/}}:
share files, collaborate, store assets, IPFS as infrastructure, lower your storage usage, decentralise your data, build a dApp, decentralise the Web itself, Blockchain use-cases, decentralised identity, ...

% \subsection{File Hosting and Data Synchronization}
% One of the obvious applications and use cases for a distributed file system is a file-hosting
% service, for which peers offer their free storage space to other peers in the network to allow
% replication and synchronization among multiple devices, similar to \emph{Dropbox} or \emph{Google
% Drive}. However, as mentioned, there is a lack of long-term incentives for users to participate in
% such a network.

% A project which tackles this problem is \emph{Filecoin}~\cite{Filecoin17}, a cryptocurrency that
% rewards peers that participate in the IPFS network and provide unused storage space with tokens that
% can be exchanged for other currencies or services. To verify benevolent participation, Filecoin uses
% \emph{Proof-of-Replication} and \emph{Proof-of-Spacetime}, allowing a peer to prove that they have
% replicated the file to their physical storage, and for a specific period of time. Analogous to that,
% misbehavior is penalized by deducting credits from the host's security deposit and rewards.
% \yiannis{This is what is commonly called the filecoin-IPFS integration. It is a very interesting topic, but requires quite some description and several issues to be taken into account. Another issue that comes up with Filecoin integration is the concept of a decentralised CDN, where there are delivery guarantees (i.e. the retrieval markets). I wouldn't mind referring here, although it will likely mean that we'll need more space to address it properly.}

% However, there are also applications that do not offer any direct incentives; instead, running an
% IPFS node is mandatory for using the offered service, where the service represents the incentive. An
% example for this is \emph{Textile Photos}: running their desktop or mobile app automatically makes
% the user an IPFS node with a constrained set of tasks, so that the app does not consume too many
% resources. In return, Textile provides users means to securely synchronize photos between multiple
% devices and to share them with others in a decentralised manner. Another project that incentivizes
% users to host a node for participation is \emph{OpenBazaar}, which is an open marketplace to sell
% and buy products. The service runs on top of multiple P2P networks, one of which is IPFS, so that no middle
% man and no fees are required when trading items. In this case, the P2P systems are used to host the
% stores, whereas the incentives are not having to pay any fees when making purchases or selling as
% well as having more privacy and stronger anonymity due OpenBazaar's flexibility regarding the
% individual networking components. However, combining both incentive schemes may be encouraging user
% participation even further. 

% Moreover, other projects integrated IPFS as means to store Web data, such as \emph{Neocities} or
% \emph{InterPlanetary Wayback} (IPWB)~\cite{Kelly16}.
% Neocities aims at bringing back the experience
% of surfing the Web on personalized and individual webpages with static content from the early days
% of the Web, for which IPFS is used to assist its CDN in terms of web content delivery. 
% Similarly, 

For instance, the \emph{InterPlanetary Wayback} (IPWB)~\cite{Kelly16} replicates Web data to 
support the availability of website content, which also includes
archiving of websites. Their prototype shows how the time for data dissemination scales linearly
with the number of files in IPFS~\cite{Kelly16}, which indicates that there is room for improvement
in terms of performance.

% Orbit Chat
% PeerPad

% \subsection{Video Streaming}
% \label{sub:video}

% Video traffic accounts for a significant portion of today's Internet traffic~\cite{Labovitz10},
% therefore video streaming is yet another application that can potentially benefit from using the
% distributed file storage that IPFS offers. \emph{DTube} is one such project, which provides a video
% streaming platform that is connected to the \emph{Steem} blockchain around which an ecosystem with
% platforms for blogging and social media is built. Steem enables monetization of user-created content
% by allowing curation through other users, which influences the value of the content and thus
% incentivizes users to contribute meaningful content. On DTube, the metadata and curation information
% is decentrally stored in the Steem blockchain, whereas the video files are stored in IPFS. Overall,
% this is similar to the YouTube architecture in which Google accounts can be used for multiple
% services, however, both content as well as personal data is stored centrally on Google servers.

% Thus, DTube shows a promising decentralised video streaming approach as an alternative to YouTube,
% since it provides features that are very similar to YouTube and has a fairly large and active user
% base due to the Steem ecosystem.
% \yiannis{As far as I know DTube is not using the public IPFS network. We need to refer to that and explain what is the difference and what are the implications, advantages, disadvantages. Issues that could be discussed here could relate to what they do to overcome the caching issues we discussed earlier.}
% \subsection{Placeholder}
% \hl{TODO: other apps}

==> sections/archive/NOT-USED-literature-expanded.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{IPFS in Research Studies}
\label{sec:related-work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \viet{Not completely done yet, just writing things down as I go through the literature. Will have
% to cut and condense this in later iterations.

% Many solutions seem to not differentiate/define the openness of their IPFS infrastructure despite
% handling sensitive data; hashes are stored in a (permissioned) blockchain, so only ``security by
% obscurity'' (attackers not knowing the hashes), often not even specifically encrypted, potential
% privacy implications?}

\jo{Pass over literature as discussed in call}


In the past, several studies investigated and built on top of IPFS for various purposes, with the
primary use case being an off-chain storage for blockchain applications. We provide a brief review
of the published literature in order to motivate further research in areas that have not been
covered yet.




\textbf{Web}
Sicilia et al.~\cite{DBLP:conf/mtsr/SiciliaAB16} propose a prototype that publishes Linked Open Data
(LOD) over IPFS; LOD describes structured data on the Web, which is interlinked in form of a graph,
and allows machines to read and semantically process the data. While they find IPFS to be suitable
for deployment, they highlight that adopting IPFS will inherit the properties and features of the
P2P network, which we discuss in~\autoref{sec:properties}.

Cochez et al.~\cite{DBLP:conf/icdcs/CochezHD17} similarly discuss the deployment of Linked Data and
knowledge objects on top of IPFS for the Semantic Web. The concept of triples, which represent the
relationship between two nodes in a labeled graph of Linked Data, are carried over to IPFS, where
the Merkle DAG links objects between each other.



\textbf{IoT}
Confais et al.~\cite{DBLP:conf/icfec/ConfaisLP17} adjust the IPFS protocol for the storage of IoT
application data within a fog and edge computing infrastructure. As lookups in the global DHT
involve overhead in terms of access time and network traffic, they split their infrastructure into
local sites, so that DHT lookups are only required for intra-site communication. They find improved
reading and writing speeds for their local-site scale-out NAS proposal, compared to centralised
cloud infrastructures or the default IPFS at the fog level. The authors further present another
approach~\cite{DBLP:conf/globecom/ConfaisPL18}, in which they replace the DHT by a tree-based
structure for fog computing infrastructure. They evaluate their approach by using IPFS and its
Kademlia DHT as a comparison, finding that their proposal is able to locate stored objects in less
than 15~ms, which is faster by 20\%.

Krejci et al.~\cite{DBLP:conf/esocc/KrejciS020} present another method to securely distribute IoT
data. IoT devices connect to a middleware, which leverage two channels to share data: one channel
based on MQTT for real-time data distribution which does not consider data integrity, and one
channel based on Ethereum plus IPFS which guarantees integrity. They test and compare the delays
(i.e., delays between a new data item being created and it being received by a user) of the two
channels. They find that adding integrity mechanisms increases the delays by multiple seconds, up to
a few minutes depending on the number of data sources (up from a few hundreds of milliseconds for
the real-time channel), indicating that a significant tradeoff between delay and integrity/trust.





\textbf{Blockchain}
Ali et al.~\cite{DBLP:conf/iot/AliDA17} leverage IPFS as a file storage for IoT data, along with a
blockchain for decentralised access control. Their proposed architecture uses a consortium network,
which consists of multiple sidechains for different IoT use cases to improve scalability. Encrypted
IoT data is stored on IPFS, with the hash identifier being stored on a blockchain and smart
contracts regulating the access to the IoT data.

Chen et al.~\cite{DBLP:conf/bigdataconf/ChenLLZ17} propose new storage schemes for IPFS, which
leverage blockchain to differentiate between hot and cold data to improve BitSwap along with
throughput and reliability.

Zheng et al.~\cite{DBLP:conf/webi/ZhengLCD18} discuss the consistently growing volume of
blockchains. They propose a model (at the example of Bitcoin) in which miners of a block deposit and
outsource the transaction data to IPFS. As such, only the resulting IPFS hash identifiers are added
to the blockchain to reduce the amount of added data.

Similarly, Norvill et al.~\cite{DBLP:conf/ithings/NorvillPSC18} propose a model to reduce the chain
size of Ethereum. Contract creation transactions, which carry code for creating and running smart
contracts, are moved off-chain in order to reduce the size of the chain. Instead of the code, the
transactions contain opcodes followed by IPFS file hashes, which are then retrieved from IPFS,
verified, and executed.



\textbf{Social Network}
Tenorio-Forn\'es et al.~\cite{DBLP:conf/mobisys/Tenorio-FornesH18} present a framework of an open
distributed system, which uses IPFS for data representation and distribution and in which agents
only have partial information of the system. They implement a Q\&A system, in which questions,
answers, and ratings are stored and distributed through IPFS. Data is discovered through search
agents, which will return content identifiers to data that matches the search query; data trust is
achieved by using public key cryptography. The authors suggest the use of blockchain as a
communication infrastructure is stronger consistency models are required. However, they also mention
the challenges of IPFS in terms of privacy and sustainability, and that sybil and generation attacks
need to be taken into account with their framework.

Xu et al.~\cite{DBLP:conf/icpads/XuSGL18} use Ethereum in conjunction with IPFS to build a
decentralised social network, inspired by Twitter. The authors use IPFS exclusively as storage for
videos and images; these files are stored to and fetched from IPFS by the application's frontend.
The resulting hashes are stored in the smart contract of the respective user, which carries the main
features of the social networking system.


\textbf{Publication Process}
Tenorio-Forn\'es et al.~\cite{DBLP:conf/hicss/Tenorio-FornesJ19} combine IPFS and blockchain
technologies in a prototype to decentralise the scientific publication process, while keeping the
peer-review process at the same time. Their system is built on top of IPFS in order to provide open
access to publications in a decentralised manner, moving away from traditional centralised
publishers. On the other hand, the blockchain is used to provide a reputation (and incentive) system
for reviewers and simultaneously enables transparency and accountability within the peer-review
process.


\textbf{Version Control}
Nizamuddin et al.~\cite{DBLP:journals/cee/NizamuddinSAAR19} leverage smart contracts and IPFS to
provide version control and document sharing between collaborating users. Active and previous
iterations of the document are stored on IPFS, with smart contracts being used to approve and track
changes of the document by storing the respective IPFS hashes.




\textbf{Deep Learning}
Haque~\cite{DBLP:conf/icoin/HaqueGM20} present an approach which leverages IPFS as a data storage to
enable decentralised transfer learning through smart contracts on a private blockchain. Trained
models are encrypted before being stored to IPFS; the smart contracts manage the access to both the
data and the models, allowing users to share models with one another.



\textbf{Healthcare}
Kumar et al.~\cite{DBLP:conf/comsnets/KumarMT20} combine IPFS with blockchain technology to
implement a system that stores medical patient data off-chain. IPFS identifiers are stored in a
consortium blockchain, to which only authorised clients have access to. Their model does not rely on
centralised third-party entities but addresses the issue of data storage in a decentralised way.

Similarly, Sun et al.~\cite{DBLP:journals/access/SunYWW20} use IPFS as a storage platform for
electronic medical data and propose an encryption scheme for these medical records. The authors
describe an attribute-based encryption system, which adds access control and authorisation
mechanisms. They integrate IPFS hashes into blockchain technology for traceability and integrity
checks of the stored files.



\textbf{Software Bugs}
Hoffman et al.~\cite{DBLP:conf/ccwc/HoffmanBMK20} introduce a bug bounty system, which they build on
top of Ethereum smart contracts and IPFS. The system is designed so that bugs are submitted to the
blockchain along with a smart contract, so that bug fixes can be issued to the contract to collect
the bounty. Bug reports and summaries for the accepted fixes are then stored off-chain on IPFS, with
the hash recorded in the blockchain.



% ACCESS CONTROL, RIGHTS MANAGEMENT, TRACEABILITY SYSTEMS/SUPPLY CHAINS, SHARING CONTROL

\textbf{Access Control, Rights Management, Traceability Systems/Supply Chains, Sharing Control}
Steichen et al.~\cite{DBLP:conf/ithings/SteichenFNSS18} discuss IPFS as storage space for large
files, which cannot be stored on blockchains. They modify IPFS and use Ethereum smart contracts to
address the lack of access control for files within IPFS. Whenever a file is being moved to/between
nodes in IPFS, their modification first checks the nodes' permissions through an access control
list, which is managed by the smart contract. Through experiments, they show that the added access
control also adds noticeable latency (multiple seconds) due to the interaction with the blockchain,
however, conclude that it is insignificant to operations. 

Ohashi et al.~\cite{DBLP:conf/blockchain2/OhashiWI0NK19} modify and enhance IPFS by integrating a
sharing control mechanism based on blockchain tokens, similar to Steichen et
al.~\cite{DBLP:conf/ithings/SteichenFNSS18}. The difference is that Ohashi et al. focus on the
blockchain tokens, rather than implementing access control through smart contracts. When adding
files to IPFS, their approach registers the file along with the token access information on both
IPFS and the blockchain, which will then be used to manage access control.

Nizamuddin et al.~\cite{DBLP:conf/icbc/NizamuddinHS18} present a solution which verifies the
integrity and authenticity of digital content by using IPFS and smart contracts. With contracts
between content creators and publishers, consumers can verify the integrity and legitimacy of their
acquired copy through the IPFS hash and the smart contract traceback.

Agyekum et al.~\cite{DBLP:conf/icig/AgyekumXLPCKYG19} combine a private IPFS network and blockchain
to propose a system that manages digital copyrights. They generate digital fingerprints of a file
and store the fingerprint (key), together with the IPFS hash and decoded metadata (value), as a
key-value pair in the blockchain. The fingerprints allow to check if uploaded files already exists,
while also keeping the size of the blockchain small. The use of a private IPFS network as storage
mechanism allows personal data to be removed from the cache of nodes, offering more flexibility than
storing it on the immutable blockchain.

Mukne et al.~\cite{DBLP:conf/icccnt/MuknePRA19} use Hyperledger Fabric and IPFS for land record
management. Files and documents associated with the land ownership are encrypted before being stored
on IPFS, so that all stakeholders can access the documents. The resulting IPFS hash is then added to
the blockchain record, so that the blockchain can provide transparency and immutability of
acquisition records.

Li et a.~\cite{DBLP:conf/blocksys/LiYHZ19} develop an authority management framework for
traceability systems, so that access to supply chains can be regulated. They use Hyperledger Fabric
to store shared information and IPFS hashes on the permissioned blockchain, with the original supply
chain data being stored on IPFS to reduce the size of the chain and to provide enhanced privacy.

Nyaletey et al.~\cite{DBLP:conf/blockchain2/NyaleteyPZC19} complement a private IPFS network with
blockchain technology in order to provide distinct audit trails. Their proposed model strengthens
trust relationships with the data by enabling tracebacks to the original author, while also tracking
access to the files by both authorised and unauthorised users. All meta and access activity data of
the file are recorded in the blockchain for traceability.




\textbf{IPFS Search Engine}
Khudhur and Fujita~\cite{DBLP:conf/ic-nc/KhudhurF19} design a decentralised search engine for IPFS.
They propose to store the associations of keywords (which can then be queried) and IPFS content
identifiers in the DHT, while simultaneously caching results of queries to speed up searches. The
search-index consists of hashes of keywords, which refers to files that contain a list of content
identifiers of files matching the keyword. The advantage of such a search-index, which is integrated
into the DHT, is that it is maintained decentrally by the P2P network and therefore has no single
point of failure. 





\textbf{Biological Data}
Zhang et al.~\cite{DBLP:conf/hucc/ZhangMHGX19} propose two migration algorithms which shard and
upload biological data to IPFS. For improved dissemination of data, the authors consider the load of
a node based on the DHT and the popularity of the data through historical access tables, which they
use to move popular data to nodes with lower load and delays.







\textbf{Performance}
Shen et al.~\cite{DBLP:conf/iwqos/ShenLZW19} investigate the I/O performance of IPFS. They deploy
IPFS storage nodes (along with HTTP servers) on Amazon EC2 servers around the globe to test and
compare the performance from a client perspective (from Tokyo, JP). They perform and measure write
operations within the local client node, as well as read operations from the local as well as remote
nodes. In order to account for different scenarios, they further test these operations for smaller
files (1--256kB), larger files (1--64~MB), and I/O traces of real online applications. They find
that read and write performance is related to the access patterns, in particular request size, as
IPFS uses different strategies for different I/O requests. They further show that for remote reads,
resolving (lookups and routing) and downloading operations can both be bottlenecks.







\textbf{VoDs, Content Retrieval, Marketplace}
Ascigil et al.~\cite{DBLP:conf/acmicn/AscigilRKP0HKK19} design a content retrieval marketplace over
IPFS, which leverages user-contributed storage space in an edge ISP for caching video content. They
compare the performance of streaming video files from IPFS with Named Data Networking (NDN), an
\ac{ICN} solution, finding that IPFS itself is not suitable to replace the role of a CDN within an
ISP. However, they also find IPFS (application layer) and NDN (network layer) to be complementing
each other regarding efficiency and scalability of routing.






\textbf{Malware, Security}
Patsakis and Casino~\cite{DBLP:journals/ijisec/PatsakisC19} investigate the use of IPFS as storage
for malware and as a means for botnet coordination. Malicious content and actors both leverage the
properties of IPFS for malicious activity, in particular anonymity, difficulty of explicit removal
from the network, content immutability, and ultimately simplicity of replication and dissemination.
The bots use algorithms that generate resource identifiers in order to receive commands, deposited
on IPFS, from the botmaster through IPFS gateways.

Casino et al.~\cite{DBLP:journals/access/CasinoPAP20} discuss challenges and threats of
decentralised file storages, in particular IPFS. The immutability properties of blockchains and
decentralised file storages such as IPFS pose threats to personal data and represent challenges
regarding distribution of illegal content, malware, as well as complications regarding update and
deprecation of outdated information. They also discuss legal issues, such as the European \ac{GDPR}
or Right to be Forgotten (cf.~\autoref{sub:persistence}).





\textbf{Measurements}
Henningsen et al.~\cite{Henningsen20} perform active and passive measurements on the public IPFS
network. They deploy modified IPFS nodes, which allows unlimited connections to other peers, and
monitor the set of incoming connections, once from behind a NAT and once from a publicly reachable
node. They further repeatedly crawl the Kademlia DHT with pre-imaged hashes to learn about all nodes
in the DHT buckets of nodes they encounter. Both measurement approaches yield on average roughly
40--45k nodes in the whole IPFS network. The authors also find that most IPFS nodes are run by
private users due to most probes announcing IP addresses in private address ranges, suggesting
symmetric NATs. As such, they observe short session times as well, indicating that the majority of
users join the IPFS network on an as-needed basis.



==> sections/archive/adoption.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Support and Adoption}
\label{sec:adoption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

IPFS is seeing increasing support and adoption by multiple projects and applications, which
indicates a high interest and potential relevance for the Future Internet. The community centered
around the open source IPFS project has witnessed a considerable growth on
\emph{Github}~\cite{FilecoinPrimer17}. Further, the close integration with Ethereum, smart contracts
and decentralised apps (so called \emph{dApps}), as well as other blockchains that use IPFS as a
decentralised storage mechanism, have influenced its growth substantially, too.

In particular, Mozilla has approved IPFS for Firefox starting from version 59 (March 2018), allowing
the community to create add-ons building on IPFS, though Firefox does not support the protocol
natively yet. As mentioned, Cloudflare has further deployed IPFS gateways in more than 150 of their
data centers, aiming to provide ''end-to-end integrity'' through the fingerprints while supporting
the growth of the IPFS ecosystem. According to Filecoin~\cite{FilecoinPrimer17}, more than 5 billion
files are hosted on IPFS as of July 2017, with the \texttt{ipfs.io} gateway experiencing up to 500
GB of daily HTTP traffic and 16 million requests. 
Due to the growing support, we envision IPFS to play a significant role in defining the Future
Internet.


% Integrated in Textile as mentioned, wants to add 1 million nodes

==> sections/literature-condensed.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{IPFS in Research Studies and Existing Applications}
\label{sec:related-work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Considering the presented properties of IPFS, it has gained attention and usage in both academic and industrial projects. We provide an overview of previous research studies and existing applications to highlight use cases of IPFS.

\subsection{Research Studies}
% Many solutions seem to not differentiate/define the openness of their IPFS infrastructure despite
% handling sensitive data; hashes are stored in a (permissioned) blockchain, so only ``security by
% obscurity'' (attackers not knowing the hashes), often not even specifically encrypted, potential
% privacy implications?}

Several studies investigated and built on top of IPFS as a main component of their proposal for
various purposes, with the primary use case being an off-chain storage for blockchain and other
decentralised applications. We provide a brief review of the published literature in order to
motivate further research on applications and areas that have not been covered yet. For instance,
most approaches rely heavily on distributed ledger technologies to implement access control and
trust mechanisms, whereas other properties of IPFS such as the best-effort storage have not been
addressed yet at all.




\textbf{Linked Data and Semantic Web.}
Studies~\cite{DBLP:conf/mtsr/SiciliaAB16,DBLP:conf/icdcs/CochezHD17} proposed the publication of
Linked Data on top of IPFS as an extension to the Semantic Web. Objects in IPFS are structured and
linked in a DAG, which translates well to the graph structure of linked data, as the relationships
between objects allow machines to read and semantically process data.


\textbf{Storage for IoT applications.}
IoT devices generate large volumes of data, which usually are sent and processed in cloud and edge
infrastructure. Previous
studies~\cite{DBLP:conf/iot/AliDA17,DBLP:conf/icfec/ConfaisLP17,DBLP:conf/esocc/KrejciS020}
presented approaches in which IPFS is used as storage for IoT applications. As lookups in the DHT,
are slow, in particular the global IPFS DHT,
studies~\cite{DBLP:conf/icfec/ConfaisLP17} showed how reducing the
number of lookups by building local clusters or even replacing the DHT with a tree-based structure
can result in locating stored objects in less than 15~ms. Other
studies~\cite{DBLP:conf/iot/AliDA17,DBLP:conf/esocc/KrejciS020} suggested to incorporate IPFS and
blockchains into IoT storage solutions in order to add trust, access control, and confidentiality.
However, there is a performance tradeoff, as adding trust increases delays by up to a few seconds or
even minutes~\cite{DBLP:conf/esocc/KrejciS020}.


\textbf{Reducing blockchain size.}
Due to the append-only nature, the size of a blockchain can only increase over time. Proposed
models~\cite{DBLP:conf/webi/ZhengLCD18,DBLP:conf/ithings/NorvillPSC18} outsource the transaction and
smart contract data to IPFS, while the blockchains only hold the IPFS hashes in order to reduce the
size of appended blocks. The stored hashes can then be used to retrieve the respective data from
IPFS, e.g., for transaction validation or contract execution.


\textbf{Wisdom of the crowd.}
IPFS was used in conjunction with Ethereum to build a decentralised online social
network~\cite{DBLP:conf/icpads/XuSGL18}: Videos and images were stored on IPFS, whereas the main
features of the system ran on top of Ethereum smart contracts. Similarly, another
study~\cite{DBLP:conf/hicss/Tenorio-FornesJ19} presented a prototype for a decentralised scientific
publication process on top of IPFS and a blockchain, where IPFS is used to openly access the papers.
On the other hand, the blockchain represents a reputation and incentive system for the reviewers,
while also enabling transparency and accountability in the review process. A framework for a Q\&A system was
presented in \cite{DBLP:conf/mobisys/Tenorio-FornesH18} (cf. \emph{StackOverflow}).
% The authors discuss open challenges of IPFS in terms of privacy and sustainability, and that sybil
% and generation attacks need to taken into consideration. 
The proposed framework includes search agents to discover questions and answers among the IPFS nodes;
a decentralised search engine for IPFS was similarly proposed in ~\cite{DBLP:conf/ic-nc/KhudhurF19}: it builds a search-index which consists of hashes of
keywords, with the associations of keywords being integrated into the DHT to enable decentralised
searches.


\textbf{Healthcare systems.}
In medical environments, the integrity of healthcare records is an essential property for patient
treatment, along with confidentiality, access control, and authorisation. Several
studies~\cite{DBLP:conf/iccsp/WuD19,DBLP:conf/comsnets/KumarMT20,DBLP:journals/access/SunYWW20}
aim to build systems that allow distribution of medical records (e.g., between physicians) in a secure
manner. To achieve this, they leverage permissioned blockchains and encryption schemes stored on
IPFS to guarantee that only authorised parties have access to patient and medication data. This
further allows traceability and integrity checks for the stored data.


\textbf{Access control, auditing, and supply chains.}
Various
studies~\cite{DBLP:conf/ithings/SteichenFNSS18,DBLP:conf/blockchain2/OhashiWI0NK19,DBLP:conf/blocksys/LiYHZ19,DBLP:conf/blockchain2/NyaleteyPZC19}
develop access control and authorisation mechanisms for IPFS storage in combination with blockchain
solutions. One proposal builds on top of smart contracts and access control
lists~\cite{DBLP:conf/ithings/SteichenFNSS18}, while another
one~\cite{DBLP:conf/blockchain2/OhashiWI0NK19} leverages blockchain tokens to achieve access
control. A proposed authority management framework~\cite{DBLP:conf/blocksys/LiYHZ19} allows to trace
access supply chain data, which is outsourced to IPFS to reduce the blockchain size. Similarly,
blockchains can be used to provide distinct audit trails for files within a private IPFS
network~\cite{DBLP:conf/blockchain2/NyaleteyPZC19}, logging every access to the file to allow
tracing back to its original author among other properties; a related approach leverages IPFS and
blockchains to provide integrity checks and access logs for data on cloud storage~\cite{Hasan19}.

% \textbf{Digital rights management.} Other papers presented systems that manage digital
% copyrights~\cite{DBLP:conf/icbc/NizamuddinHS18,DBLP:conf/icig/AgyekumXLPCKYG19,Shi19} to
% facilitate an ecosystem for creators, publishers, and consumers. The transparency property of
% blockchains as well as the unique content identifiers of IPFS allow clients to verify the
% integrity and authenticity of files, while simultaneously revealing file duplication.

% \textbf{Malware and security.}
% As a decentralised file storage, IPFS faces a variety of challenges and security
% threats~\cite{DBLP:journals/access/CasinoPAP20}. The immutability properties of blockchains and IPFS
% pose threats to personal data and represent challenges, which we have already discussed partially
% in~\autoref{sub:persistence}. Among others, distribution of illegal content and malware,
% complications w.r.t. update and deprecation of outdated information, and legislations such as the
% European \ac{GDPR} or Right to be Forgotten represent open research questions and challenges for
% IPFS. For instance, as files cannot be explicitly removed from the network, IPFS is used as storage
% for malware and as a means for botnet coordination: Bots use algorithms that deterministically
% generate resource identifiers in order to receive commands, deposited on IPFS, from the botmaster
% through IPFS gateways~\cite{DBLP:journals/ijisec/PatsakisC19}.


\textbf{Performance and topology measurements.}
To study the performance of IPFS, a study performed measurements from local and remote
nodes~\cite{DBLP:conf/iwqos/ShenLZW19}. The authors found that read and write performance of clients
is related to access patterns, in particular request size, since IPFS uses different strategies for
different I/O requests. They also showed that for remote reads, resolving (lookups, routing) and
downloading operations can both be performance bottlenecks.

A study on the IPFS topology~\cite{Henningsen20} used a modified IPFS node, which accepted unlimited
connections from other peers, to collect passive measurements of the P2P network. They further
repeatedly scraped the DHT in order to actively measure the number of connected nodes; both
measurement approaches yield on average roughly 40--45k nodes in the whole IPFS network. They found
that most probes are run by private users behind symmetric NATs, with short-lived sessions, which
indicates that most clients join the IPFS network on an as-needed basis.


\textbf{Other use cases.}
IPFS was further used to enable a variety of other applications and use cases, which we cannot
discuss in detail for the sake of brevity. Instead, we provide a brief list of other use
cases/studies (in no particular order) which have built on top of IPFS: alternative storage schemes
for IPFS~\cite{DBLP:conf/bigdataconf/ChenLLZ17}, verifiable voting
systems~\cite{DBLP:conf/ithings/PerezC18}, collaborative document editing with version
control~\cite{DBLP:journals/cee/NizamuddinSAAR19}, land record
management~\cite{DBLP:conf/icccnt/MuknePRA19}, digital right
management~\cite{DBLP:conf/icbc/NizamuddinHS18,DBLP:conf/icig/AgyekumXLPCKYG19,Shi19}, content
retrieval marketplaces~\cite{DBLP:conf/acmicn/AscigilRKP0HKK19}, training of federated learning
models~\cite{Liu19}, exchange of decentralised transfer learning
models~\cite{DBLP:conf/icoin/HaqueGM20}, software integrity and delivery
frameworks~\cite{DBLP:conf/icgse/SingiKBP19}, bug bounty system~\cite{DBLP:conf/ccwc/HoffmanBMK20},
biological data migration~\cite{DBLP:conf/hucc/ZhangMHGX19}, among others.




\subsection{Existing Applications Built on IPFS}

Various applications build on top of IPFS in order to decentralise the application storage and to avoid having to trust a single storage provider. The complexity of the applications and the role of IPFS within the projects differ based on the use cases, which range from using IPFS as infrastructure for file sharing and asset storage (e.g., for Web applications) to supply chain networks and data aggregation platforms, among others. These projects leverage the strengths of IPFS regarding content addressing (for deduplication and integrity checks) as well as P2P storage in particular. We present a few selected examples to showcase the versatility of IPFS in decentralised applications.

\textbf{Web Tools: Building, Hosting, Deploying on IPFS.}
Textile\footnote{\url{https://textile.io/}} and Fleek\footnote{\url{https://fleek.co/}} build tools on top of IPFS, which facilitate moving or migrating Web content and applications towards a decentralised Web. They
% provided interfaces, integrations, and pipelines
allow developers to easily move their website or Web service from a local development branch to a deployment environment based on IPFS:
Instead of deploying a site on a centralised host, a site and its assets are stored and deployed on the decentralised IPFS network, which in return provides the properties discussed in~\autoref{sec:properties}. 

\textbf{Data Management and Archival.}
% The content-addressed naming scheme of IPFS provides inherent deduplication and links between related IPFS object pieces, along with built-in integrity validation.
The inherent integrity validation, deduplication, and links between related IPFS objects are leveraged by data management systems, as offered by Qri\footnote{\url{https://qri.io/}} or OrbitDB\footnote{\url{https://orbitdb.org/}}, which build decentralised databases. Based on IPFS, these databases provide versioning, logging, synchronisation, and sharing of data in a decentralised manner, while also supporting mutable content, which is particularly useful for decentralised applications: \emph{QRI} builds an overlay P2P network on top of IPFS and allows its users to share datasets among each other and track changes through version control features, essentially providing a dynamic, distributed database. \emph{OrbitDB} provides eventual consistency through conflict-free replicated data types (CRDTs). Similarly, \emph{Ceramic} uses smart documents which leverage IPFS and other decentralised approaches, such as Decentralised Identifiers (DIDs) and blockchains, to store mutable content (referred to by unique and immutable identifiers) in a censorship-resistant network.

Another project that leverages IPFS' file system properties is the InterPlanetary Wayback (IPWB)~\cite{Kelly16}. Contrary to its centralised ``counterpart'' of the Wayback Machine, IPWB distributes the archived content among multiple peers in the P2P network, which uses the deduplication properties of IPFS to reduce the amount of space required for Web archival.

% Qri provides a version control and sharing system for structured datasets, building on top of IPFS, which allows it to check the authenticity and integrity of data along with file changes thanks to its content addressing properties.

\textbf{Pinning Services.}
As mentioned in~\autoref{sub:incentives}, pinning services such as Pinata\footnote{\url{https://pinata.cloud/}} or Temporal\footnote{\url{https://temporal.cloud/}} run dedicated IPFS nodes that keep content persistent in the IPFS network, typically in exchange for a fee. This improves the availability of the pinned objects, as the pinned content will be less affected by churn or other losses of connectivity thanks to the distributed replication of the pinning services. As such, these services can be used as a complement or alternative to cloud hosts or \acp{CDN} for purposes of data storage and retrieval.

\textbf{E-Commerce and Marketplaces.} In the OpenBazaar\footnote{\url{https://openbazaar.org/}} P2P network, sellers host online shops on IPFS to store shop assets and product information. The properties of IPFS also allow sellers to have full control over which items they decide to list, i.e., what information they would like to publish. Buyers can connect to sellers directly, meaning that no platform fees are charged by a centralised third party. The IPFS network assists in caching content among users, so shops can continue to function while the main seller's IPFS node is offline. Different search engines (which the user can freely choose) enable the discovery of items, allowing users to find items by searching for keywords provided by the sellers.
% The payment system is based on cryptocurrencies; users can act as trusted moderators on the network, i.e., they can resolve potential disputes between buyers and sellers (e.g., refunding payments that were transferred to an escrow account), for which the moderator receives a fraction of the transaction fee after solving the dispute.
Similar concepts are adopted by Origin\footnote{\url{https://www.originprotocol.com/; e-commerce}} and Filehive\footnote{\url{https://filehive.app/; dataset marketplace}}.

Arbol\footnote{\url{https://www.arbolmarket.com/}} builds a risk marketplace for weather-related risks on top of IPFS and blockchain-based contracts. The Arbol platform aggregates longitudinal weather data from multiple sources and stores them on IPFS. These datasets can then be used as reliable information to verify contracts between weather-dependent stakeholders concerning protection agreements.
% ; for instance, the platform minimises the risks for farmers or other agricultural entities which are not able to harvest the agreed upon amounts of products due to bad weather conditions, which can be proven by the decentralised data and transparent contract.


\textbf{Digital Content Sharing.} In order to provide decentralised music streaming, Audius\footnote{\url{https://audius.org/}} combines IPFS and blockchain to give music artists full control over their content. The metadata and audio files are stored and delivered through the decentralised IPFS network, whereas the blockchain is used for content registration and access management through a token economy. Artists use content nodes to publish (encrypted) content on the IPFS network along with a smart contract on the blockchain, which listeners can unlock through a smart contract mechanism. The encrypted content can be retrieved from IPFS at any time, however, conditions for unlocking the content can be defined by the artist, e.g., by payment or by proving the possession of sufficient tokens of the artist.
% After the conditions are met and proven to the content node (operated or trusted by the publishing artist), the content node derives a re-encryption key specific to the requesting listener, with which the listener can locally re-encrypt and finally decrypt the requested segment of a music track for streaming.
The ledger provides transparency to both artists and other listeners regarding listening behavior.

% Similarly, LikeCoin\footnote{\url{https://like.co/}} represents a digital publishing infrastructure that operates on decentralised registries and rewards. Content pieces and their metadata, which includes their IPFS content addresses, are assigned a unique identifier (cf. ISBN) that is stored on a blockchain. The use of IPFS for content storage and retrieval makes the content immutable, verifiable, and censorship-resistant. Consumers that ``like'' the (freely available) content will provide rewards (LikeCoin tokens) to the publishers. 


% \textbf{Supply Chain Network.}
% Morpheus.Network\footnote{\url{https://morpheus.network/}} uses a private IPFS network to store and retrieve shipping documentation in a distributed and verifiable manner to build a supply chain platform. It further uses the Ethereum blockchain and a private sidechain to log transactions and events (along with the IPFS CIDs of related documents) in the shipping process, while the shipping-related documents are stored in an encrypted form on the private IPFS network; this private IPFS network allows Morpheus.Network to persist files indefinitely through pinning. The supply chain platform acts as an interfaces to this private IPFS network, whereas the content-addressing properties of IPFS allow verification of the retrieved document based on the event logs and cryptographic hashes. Although this verification would be possible without IPFS, IPFS facilitates the storage and retrieval of the shipping documents and improves the usability of the system, without having to compromise on trust.


% Note: List below only contains projects that are still somewhat actively maintained and developed

% Orion (classic ile sharing)

% Berty.Tech (messaging, offline + online)

% Decentraland (VR assets)

% Qri (data management), OrbitDB (decentralised database)

% Killcord (deadman switch)

% Fission/Fleek (video live-streaming)

% KODA: Koda-9 (decentralised robot dog)

% Actyx (Industry 4.0, OS on top of IPFS for sync and coordination)

% Textile (hosting on top of IPFS)

% Fleek (deployment pipelines to build website/app on IPFS)

% Origin (online commerce platform), Filehive, OpenBazaar

% Decentralised BitTorrent trackers (avoid single point of failure)

% Audius (music streaming)

% Aragon (decentralised autonomous organizations)

% InterPlanetary Wayback (web archiving, see paper~\cite{Kelly16})

% IOTA (IPFS as storage for data for IOT data)

% MindSync (blockchain for AI as a service, AI competitions)

% Robonomics (exchange smart city data)

% Augur (online betting)

% Arbol (weather data verification + risk marketplace)

% Ceramic (decentralised identity)

% LikeCoin (content publishing, immutable content metadata)

% Morpheus.Network (supply chain platform)
